Thermoelectric study of dissipative quantum dot heat engines

This paper examines the thermoelectric response of a dissipative quantum dot heat engine based on the Anderson-Holstein model in two relevant operating limits: (i) when the dot phonon modes are out of equilibrium, and (ii) when the dot phonon modes are strongly coupled to a heat bath. In the first case, a detailed analysis of the physics related to the interplay between the quantum dot level quantization, the on-site Coulomb interaction and the electron-phonon coupling on the thermoelectric performance reveals that an n-type heat engine performs better than a p-type heat engine. In the second case, with the aid of the dot temperature estimated by incorporating a {\it{thermometer bath}}, it is shown that the dot temperature deviates from the bath temperature as electron-phonon interaction becomes stronger. Consequently, it is demonstrated that the dot temperature controls the direction of phonon heat currents, thereby influencing the thermoelectric performance. Finally, the conditions on the maximum efficiency with varying phonon couplings between the dot and all the other macroscopic bodies are analyzed in order to reveal the nature of the optimum junction.

==> physics.sty.tex <==
\ProvidesPackage{physics}
% physics 1.3
% This material is subject to the LaTeX Project Public License.
% See http://www.ctan.org/tex-archive/help/Catalogue/licenses.lppl.html for the details of that license.
%
% Handy commands for physicists including macros for vectors, calculus, matrices, and bra-ket (Dirac) notation
% Requires xparse package, which comes bundled with l3packages and l3kernel
% This package loads amsmath, which comes standard with most latex distributions
% The commands defined in this package will silently overwrite previous commands with the same name, if such commands exist
%
% Created by Sergio C. de la Barrera
% Updated on December 12, 2012
% Uploaded on December 20, 2012

\RequirePackage{xparse}
\RequirePackage{amsmath}

% Options
\DeclareOption{trig}{\let\trigopt = 1}
\DeclareOption{notrig}{\let\trigopt = 0}
\DeclareOption{uprightdiff}{\def\diffd{\mathrm{d}}} % Upright differentials
\DeclareOption{italicdiff}{\def\diffd{d}} % Italic differentials
\DeclareOption{bolddel}{\DeclareDocumentCommand\vnabla{}{\boldsymbol\nabla}} % Vector bold \nabla symbol
\DeclareOption{arrowdel}{\DeclareDocumentCommand\vnabla{}{\vec{\boldsymbol\nabla}}} % Vector arrow \nabla symbol
\ExecuteOptions{trig,uprightdiff,bolddel}
\ProcessOptions\relax

% Symbols
\ProvideDocumentCommand\varE{}{\mathcal{E}} % Curly 'E'
\ProvideDocumentCommand\ordersymbol{}{\mathcal{O}} % Order symbol --> O(x^2)
\ProvideDocumentCommand\lparen{}{(} % Left parenthesis
\ProvideDocumentCommand\rparen{}{)} % Right parenthesis

% Brackets and braces
\DeclareDocumentCommand\quantity{}{{\ifnum\z@=`}\fi\@quantity}
\DeclareDocumentCommand\@quantity{ t\big t\Big t\bigg t\Bigg g o d() d|| }
{ % Flexible automatic bracketing of an expression in () or [] or {} or ||
	% Handles manual override of sizing
	\IfBooleanTF{#1}{\let\ltag\bigl \let\rtag\bigr}{
		\IfBooleanTF{#2}{\let\ltag\Bigl \let\rtag\Bigr}{
			\IfBooleanTF{#3}{\let\ltag\biggl \let\rtag\biggr}{
				\IfBooleanTF{#4}
				{\let\ltag\Biggl \let\rtag\Biggr}
				{\let\ltag\left \let\rtag\right}
			}
		}
	}
	% Handles actual bracketing
	\IfNoValueTF{#5}{
		\IfNoValueTF{#6}{
			\IfNoValueTF{#7}{
				\IfNoValueTF{#8}
				{()}
				{\ltag\lvert{#8}\rtag\rvert}
			}
			{\ltag(#7\rtag) \IfNoValueTF{#8}{}{|#8|}}
		}
		{\ltag[#6\rtag] \IfNoValueTF{#7}{}{(#7)} \IfNoValueTF{#8}{}{|#8|}}
	}
	{\ltag\lbrace#5\rtag\rbrace  \IfNoValueTF{#6}{}{[#6]} \IfNoValueTF{#7}{}{(#7)} \IfNoValueTF{#8}{}{|#8|}}
	\ifnum\z@=`{\fi}
}
\DeclareDocumentCommand\qty{}{\quantity} % Shorthand for \quantity
\DeclareDocumentCommand\pqty{ l m }{\braces#1{\lparen}{\rparen}{#2}}
\DeclareDocumentCommand\bqty{ l m }{\braces#1{\lbrack}{\rbrack}{#2}}
\DeclareDocumentCommand\Bqty{ l m }{\braces#1{\lbrace}{\rbrace}{#2}}
\DeclareDocumentCommand\vqty{ l m }{\braces#1{\lvert}{\rvert}{#2}}


\DeclareDocumentCommand\pmqty{m}{\begin{pmatrix}#1\end{pmatrix}}
\DeclareDocumentCommand\Pmqty{m}{\left\lgroup\begin{matrix}#1\end{matrix}\right\rgroup}
\DeclareDocumentCommand\bmqty{m}{\begin{bmatrix}#1\end{bmatrix}}
\DeclareDocumentCommand\vmqty{m}{\begin{vmatrix}#1\end{vmatrix}}
\DeclareDocumentCommand\matrixquantity{}{{\ifnum\z@=`}\fi\@matrixquantity}
\DeclareDocumentCommand\@matrixquantity{ s g o d() d|| }
{
	\mathord{
	\IfNoValueTF{#2}
	{
		\IfNoValueTF{#3}
		{
			\IfNoValueTF{#4}
			{
				\IfNoValueTF{#5}
				{()}
				{\vmqty{#5}}
			}
			{
				\IfBooleanTF{#1}
				{\Pmqty{#4}}
				{\pmqty{#4}}
				\IfNoValueTF{#5}{}{|#5|}
			}
		}
		{\bmqty{#3} \IfNoValueTF{#4}{}{(#4)} \IfNoValueTF{#5}{}{|#5|}}
	}
	{\begin{matrix}#2\end{matrix} \IfNoValueTF{#3}{}{[#3]} \IfNoValueTF{#4}{}{(#4)} \IfNoValueTF{#5}{}{|#5|}}
	}
	\ifnum\z@=`{\fi}
}
\DeclareDocumentCommand\mqty{}{\matrixquantity} % Shorthand for \matrixquantity
\DeclareDocumentCommand\matrixdeterminant{m}{\vmqty{#1}} % Matrix determinant
\DeclareDocumentCommand\mdet{}{\matrixdeterminant} % Shorthand for matrix determinant

\DeclareDocumentCommand\spmqty{m}{\pqty{\begin{smallmatrix}#1\end{smallmatrix}}}
\DeclareDocumentCommand\sPmqty{m}{\left\lgroup\begin{smallmatrix}#1\end{smallmatrix}\right\rgroup}
\DeclareDocumentCommand\sbmqty{m}{\bqty{\begin{smallmatrix}#1\end{smallmatrix}}}
\DeclareDocumentCommand\svmqty{m}{\vqty{\begin{smallmatrix}#1\end{smallmatrix}}}
\DeclareDocumentCommand\smallmatrixquantity{ s g o d() d|| }
{
	\mathord{
	\IfNoValueTF{#2}
	{
		\IfNoValueTF{#3}
		{
			\IfNoValueTF{#4}
			{
				\IfNoValueTF{#5}
				{()}
				{\svmqty{#5}}
			}
			{
				\IfBooleanTF{#1}
				{\sPmqty{#4}}
				{\spmqty{#4}}
				\IfNoValueTF{#5}{}{|#5|}
			}
		}
		{\sbmqty{#3} \IfNoValueTF{#4}{}{(#4)} \IfNoValueTF{#5}{}{|#5|}}
	}
	{\begin{smallmatrix}#2\end{smallmatrix} \IfNoValueTF{#3}{}{[#3]} \IfNoValueTF{#4}{}{(#4)} \IfNoValueTF{#5}{}{|#5|}}
	}
}
\DeclareDocumentCommand\smqty{}{\smallmatrixquantity} % Shorthand for \smallmatrixquantity
\DeclareDocumentCommand\smallmatrixdeterminant{m}{\svmqty{#1}} % Small matrix determinant
\DeclareDocumentCommand\smdet{}{\smallmatrixdeterminant} % Shorthand for small matrix determinant

\DeclareDocumentCommand\argopen{s}{\IfBooleanTF{#1}{\mathopen{}\mathclose\bgroup}{\mathopen{}\mathclose\bgroup\left}} % Special open grouping for argument of a function
\DeclareDocumentCommand\argclose{s}{\IfBooleanTF{#1}{\egroup}{\aftergroup\egroup\right}} % Special close grouping for argument of a function

\DeclareDocumentCommand\braces{}{{\ifnum\z@=`}\fi\@braces}
\DeclareDocumentCommand\@braces{ s t\big t\Big t\bigg t\Bigg m m m }
{ % General braces with automatic and manual sizing
	\IfBooleanTF{#1}
	{\left#6\smash{#8}\right#7\vphantom{#8}}
	{
		\IfBooleanTF{#2}{\bigl#6{#8}\bigr#7}{
			\IfBooleanTF{#3}{\Bigl#6{#8}\Bigr#7}{
				\IfBooleanTF{#4}{\biggl#6{#8}\biggr#7}{
					\IfBooleanTF{#5}{\Biggl#6{#8}\Biggr#7}{\left#6{#8}\right#7}
				}
			}
		}
	}
	\ifnum\z@=`{\fi}
}

\DeclareDocumentCommand\fbraces{ s t\big t\Big t\bigg t\Bigg m m m m }
{ % Function braces with automatic and manual sizing
	#8
	\IfBooleanTF{#1}
	{\argopen#6\smash{#9}\argclose#7\vphantom{#9}}
	{
		\IfBooleanTF{#2}{\argopen*\bigl#6{#9}\argclose*\bigr#7}{
			\IfBooleanTF{#3}{\argopen*\Bigl#6{#9}\argclose*\Bigr#7}{
				\IfBooleanTF{#4}{\argopen*\biggl#6{#9}\argclose*\biggr#7}{
					\IfBooleanTF{#5}
					{\argopen*\Biggl#6{#9}\argclose*\Biggr#7}
					{\argopen#6{#9}\argclose#7}
				}
			}
		}
	}
}

\DeclareDocumentCommand\absolutevalue{ l m }{\braces#1{\lvert}{\rvert}{#2}} % Absolute value/complex modulus
\DeclareDocumentCommand\abs{}{\absolutevalue} % Shorthand for \absolutevalue
\DeclareDocumentCommand\norm{ l m }{\braces#1{\lVert}{\rVert}{#2}} % Norm
\DeclareDocumentCommand\order{ l m }{\fbraces#1{\lparen}{\rparen}{\ordersymbol}{#2}} % Order notation -> O(x^2)

\DeclareDocumentCommand\evaluated{ s g d[| d(| }
{ % Vertical evaluation bar
	\IfNoValueTF{#2}
	{
		\IfNoValueTF{#3}
		{
			\IfNoValueTF{#4}
				{\argopen.\vphantom{\int}\argclose\rvert}
				{\IfBooleanTF{#1}{\vphantom{#4}}{}\left(\IfBooleanTF{#1}{\smash{#4}}{#4}\vphantom{\int}\right\rvert}
		}
		{\IfBooleanTF{#1}{\vphantom{#3}}{}\left[\IfBooleanTF{#1}{\smash{#3}}{#3}\vphantom{\int}\right\rvert \IfNoValueTF{#4}{}{(#4|}}
	}
	{\IfBooleanTF{#1}{\vphantom{#2}}{}\left.\IfBooleanTF{#1}{\smash{#2}}{#2}\vphantom{\int}\right\rvert \IfNoValueTF{#3}{}{[#3|} \IfNoValueTF{#4}{}{(#4|}}
}
\DeclareDocumentCommand\eval{}{\evaluated} % Shorthand for evaluated

\DeclareDocumentCommand\poissonbracket{ l m m }{\braces#1{\lbrace}{\rbrace}{#2,#3}} % Poisson bracket [same as anti-commutator]
\DeclareDocumentCommand\pb{}{\poissonbracket} % Shorthand for \poissonbracket

% Commutators
\DeclareDocumentCommand\commutator{ l m m }{\braces#1{\lbrack}{\rbrack}{#2,#3}} % Commutator
\DeclareDocumentCommand\comm{}{\commutator} % Shorthand for \commutator
\DeclareDocumentCommand\anticommutator{ l m m }{\braces#1{\lbrace}{\rbrace}{#2,#3}} % Anticommutator [same as Poisson bracket]
\DeclareDocumentCommand\acommutator{}{\anticommutator} % Shorthand for \anticommutator
\DeclareDocumentCommand\acomm{}{\anticommutator} % Shorthand for \anticommutator

% Vector notation
\DeclareDocumentCommand\vectorbold{ s m }{\IfBooleanTF{#1}{\boldsymbol{#2}}{\mathbf{#2}}} % Vector bold [star for Greek and italic Roman]
\DeclareDocumentCommand\vb{}{\vectorbold} % Shorthand for \vectorbold

\DeclareDocumentCommand\vectorarrow{ s m }{\IfBooleanTF{#1}{\vec{\boldsymbol{#2}}}{\vec{\mathbf{#2}}}} % Vector arrow + bold [star for Greek and italic Roman]
\DeclareDocumentCommand\va{}{\vectorarrow} % Shorthand for \vectorarrow

\DeclareDocumentCommand\vectorunit{ s m }{\IfBooleanTF{#1}{\boldsymbol{\hat{#2}}}{\mathbf{\hat{#2}}}} % Unit vector [star for Greek and italic Roman]
\DeclareDocumentCommand\vu{}{\vectorunit} % Shorthand for \vectorunit

\DeclareDocumentCommand\dotproduct{}{\boldsymbol\cdot} % Vector dot product symbol
\DeclareDocumentCommand\vdot{}{\dotproduct} % Shorthand for \dotproduct [note that the command sequence \dp is protected]

\DeclareDocumentCommand\crossproduct{}{\boldsymbol\times} % Vector cross product symbol
\DeclareDocumentCommand\cross{}{\crossproduct} % Shorthand for \crossproduct
\DeclareDocumentCommand\cp{}{\crossproduct} % Shorthand for \crossproduct

\DeclareDocumentCommand\gradient{ g o d() }{ % Gradient
	\IfNoValueTF{#1}{
		\IfNoValueTF{#2}{
			\IfNoValueTF{#3}{\vnabla}{\fbraces{\lparen}{\rparen}{\vnabla}{#3}}
			}
			{\fbraces{\lbrack}{\rbrack}{\vnabla}{#2} \IfNoValueTF{#3}{}{(#3)}}
		}
		{\vnabla #1 \IfNoValueTF{#2}{}{[#2]} \IfNoValueTF{#3}{}{(#3)}}
	}
\DeclareDocumentCommand\grad{}{\gradient} % Shorthand for \gradient

\DeclareDocumentCommand\divergence{ g o d() }{ % Divergence
	\IfNoValueTF{#1}{
		\IfNoValueTF{#2}{
			\IfNoValueTF{#3}{\vnabla \vdot}{\vnabla \vdot \quantity(#3)}
			}
			{\vnabla \vdot \quantity[#2] \IfNoValueTF{#3}{}{(#3)}}
		}
		{\vnabla \vdot #1 \IfNoValueTF{#2}{}{[#2]} \IfNoValueTF{#3}{}{(#3)}}
	}
\let\divisionsymbol\div % Rename \div [division symbol] in order to free up control sequence for \divergence
\let\div\relax
\DeclareDocumentCommand\div{}{\divergence} % Shorthand for \divergence

\DeclareDocumentCommand\curl{ g o d() }{ % Curl
	\IfNoValueTF{#1}{
		\IfNoValueTF{#2}{
			\IfNoValueTF{#3}{\vnabla \cross}{\vnabla \cross \quantity(#3)}
			}
			{\vnabla \cross \quantity[#2] \IfNoValueTF{#3}{}{(#3)}}
		}
		{\vnabla \cross #1 \IfNoValueTF{#2}{}{[#2]} \IfNoValueTF{#3}{}{(#3)}}
	}

\DeclareDocumentCommand\laplacian{ g o d() }{ % Laplacian
	\IfNoValueTF{#1}{
		\IfNoValueTF{#2}{
			\IfNoValueTF{#3}{\nabla^2}{\fbraces{\lparen}{\rparen}{\nabla^2}{#3}}
			}
			{\fbraces{\lbrack}{\rbrack}{\nabla^2}{#2} \IfNoValueTF{#3}{}{(#3)}}
		}
		{\nabla^2 #1 \IfNoValueTF{#2}{}{[#2]} \IfNoValueTF{#3}{}{(#3)}}
	}

% Operators
\DeclareMathOperator{\trace}{tr} % Trace of a matrix
\DeclareMathOperator{\Trace}{Tr} % Trace of a matrix (alternate)
\DeclareMathOperator{\rank}{rank} % Rank of a matrix
\DeclareMathOperator{\erf}{erf} % Gauss error function
\DeclareMathOperator{\Residue}{Res} % Residue
\DeclareDocumentCommand\principalvalue{g}{\IfNoValueTF{#1}{\mathcal{P}}{\mathcal{P}\mathord{#1}}}
\DeclareDocumentCommand\pv{}{\principalvalue}
\DeclareDocumentCommand\PV{g}{\IfNoValueTF{#1}{\mathrm{P.V.}}{\mathrm{P.V.}\mathord{#1}}}
\let\real\Re \DeclareDocumentCommand\Re{g}{\IfNoValueTF{#1}{\operatorname{Re}}{\fbraces{\lbrace}{\rbrace}{\operatorname{Re}}{#1}}}
\let\imaginary\Im \DeclareDocumentCommand\Im{g}{\IfNoValueTF{#1}{\operatorname{Im}}{\fbraces{\lbrace}{\rbrace}{\operatorname{Im}}{#1}}}
\DeclareDocumentCommand\opbraces{ m g o d() }
{
	\IfNoValueTF{#2}
	{
		\IfNoValueTF{#3}
			{
				\IfNoValueTF{#4}
				{#1}
				{\fbraces{\lparen}{\rparen}{#1}{#4}}
			}
			{
				\fbraces{\lbrack}{\rbrack}{#1}{#3}
				\IfNoValueTF{#4}{}{(#4)}
			}
	}
	{
		\fbraces{\lbrace}{\rbrace}{#1}{#2}
		\IfNoValueTF{#3}{}{[#3]}
		\IfNoValueTF{#4}{}{(#4)}
	}
}
\DeclareDocumentCommand\trigbraces{ m o d() }
{
	\IfNoValueTF{#3}
	{#1 \IfNoValueTF{#2}{}{[#2]}}
	{#1 \IfNoValueTF{#2}{}{^{#2}} \argopen(#3\argclose)}
}

% Trig function and operator redefinitions
\ifx\trigopt 1
	\let\sine\sin \DeclareDocumentCommand\sin{}{\trigbraces{\sine}}
	\let\cosine\cos \DeclareDocumentCommand\cos{}{\trigbraces{\cosine}}
	\let\tangent\tan \DeclareDocumentCommand\tan{}{\trigbraces{\tangent}}
	\let\cosecant\csc \DeclareDocumentCommand\csc{}{\trigbraces{\cosecant}}
	\let\secant\sec \DeclareDocumentCommand\sec{}{\trigbraces{\secant}}
	\let\cotangent\cot \DeclareDocumentCommand\cot{}{\trigbraces{\cotangent}}
	
	\let\arcsine\arcsin \DeclareDocumentCommand\arcsin{}{\trigbraces{\arcsine}}
	\let\arccosine\arccos \DeclareDocumentCommand\arccos{}{\trigbraces{\arccosine}}
	\let\arctangent\arctan \DeclareDocumentCommand\arctan{}{\trigbraces{\arctangent}}
	\DeclareMathOperator{\arccosecant}{arccsc}
	\DeclareDocumentCommand\arccsc{}{\trigbraces{\arccosecant}}
	\DeclareMathOperator{\arcsecant}{arcsec}
	\DeclareDocumentCommand\arcsec{}{\trigbraces{\arcsecant}}
	\DeclareMathOperator{\arccotangent}{arccot}
	\DeclareDocumentCommand\arccot{}{\trigbraces{\arccotangent}}

	\DeclareMathOperator{\asine}{asin}
	\DeclareDocumentCommand\asin{}{\trigbraces{\asine}}
	\DeclareMathOperator{\acosine}{acos}
	\DeclareDocumentCommand\acos{}{\trigbraces{\acosine}}
	\DeclareMathOperator{\atangent}{atan}
	\DeclareDocumentCommand\atan{}{\trigbraces{\atangent}}
	\DeclareMathOperator{\acosecant}{acsc}
	\DeclareDocumentCommand\acsc{}{\trigbraces{\acosecant}}
	\DeclareMathOperator{\asecant}{asec}
	\DeclareDocumentCommand\asec{}{\trigbraces{\asecant}}
	\DeclareMathOperator{\acotangent}{acot}
	\DeclareDocumentCommand\acot{}{\trigbraces{\acotangent}}
	
	\let\hypsine\sinh \DeclareDocumentCommand\sinh{}{\trigbraces{\hypsine}}
	\let\hypcosine\cosh \DeclareDocumentCommand\cosh{}{\trigbraces{\hypcosine}}
	\let\hyptangent\tanh \DeclareDocumentCommand\tanh{}{\trigbraces{\hyptangent}}
	\DeclareMathOperator{\hypcosecant}{csch}
	\DeclareDocumentCommand\csch{}{\trigbraces{\hypcosecant}}
	\DeclareMathOperator{\hypsecant}{sech}
	\DeclareDocumentCommand\sech{}{\trigbraces{\hypsecant}}
	\let\hypcotangent\coth \DeclareDocumentCommand\coth{}{\trigbraces{\hypcotangent}}
	
	\let\exponential\exp \DeclareDocumentCommand\exp{}{\opbraces{\exponential}}
	\let\logarithm\log \DeclareDocumentCommand\log{}{\trigbraces{\logarithm}}
	\let\naturallogarithm\ln \DeclareDocumentCommand\ln{}{\trigbraces{\naturallogarithm}}
	\let\determinant\det \DeclareDocumentCommand\det{}{\opbraces{\determinant}}
	\let\Probability\Pr \DeclareDocumentCommand\Pr{}{\opbraces{\Probability}}
	\DeclareDocumentCommand\tr{}{\opbraces{\trace}}
	\DeclareDocumentCommand\Tr{}{\opbraces{\Trace}}
	\DeclareDocumentCommand\Res{}{\opbraces{\Residue}}
\else
	\DeclareMathOperator{\arccsc}{arccsc}
	\DeclareMathOperator{\arcsec}{arcsec}
	\DeclareMathOperator{\arccot}{arccot}
	
	\DeclareMathOperator{\asin}{asin}
	\DeclareMathOperator{\acos}{acos}
	\DeclareMathOperator{\atan}{atan}
	\DeclareMathOperator{\acsc}{acsc}
	\DeclareMathOperator{\asec}{asec}
	\DeclareMathOperator{\acot}{acot}
	
	\DeclareMathOperator{\csch}{csch}
	\DeclareMathOperator{\sech}{sech}
	
	\DeclareDocumentCommand\tr{}{\trace}
	\DeclareDocumentCommand\Tr{}{\Trace}
	\DeclareDocumentCommand\Res{}{\Residue}
\fi

% Quick quad text (math-mode text with \quad spacing)
\DeclareDocumentCommand\qqtext{ s m }{\IfBooleanTF{#1}{}{\quad}\text{#2}\quad}
\DeclareDocumentCommand\qq{}{\qqtext}

\DeclareDocumentCommand\qcomma{}{,\quad}
\DeclareDocumentCommand\qc{}{\qcomma}

\DeclareDocumentCommand\qif{s}{\IfBooleanTF{#1}{}{\quad}\text{if}\quad}
\DeclareDocumentCommand\qthen{s}{\IfBooleanTF{#1}{}{\quad}\text{then}\quad}
\DeclareDocumentCommand\qelse{s}{\IfBooleanTF{#1}{}{\quad}\text{else}\quad}
\DeclareDocumentCommand\qotherwise{s}{\IfBooleanTF{#1}{}{\quad}\text{otherwise}\quad}
\DeclareDocumentCommand\qunless{s}{\IfBooleanTF{#1}{}{\quad}\text{unless}\quad}
\DeclareDocumentCommand\qgiven{s}{\IfBooleanTF{#1}{}{\quad}\text{given}\quad}
\DeclareDocumentCommand\qusing{s}{\IfBooleanTF{#1}{}{\quad}\text{using}\quad}
\DeclareDocumentCommand\qassume{s}{\IfBooleanTF{#1}{}{\quad}\text{assume}\quad}
\DeclareDocumentCommand\qsince{s}{\IfBooleanTF{#1}{}{\quad}\text{since}\quad}
\DeclareDocumentCommand\qlet{s}{\IfBooleanTF{#1}{}{\quad}\text{let}\quad}
\DeclareDocumentCommand\qfor{s}{\IfBooleanTF{#1}{}{\quad}\text{for}\quad}
\DeclareDocumentCommand\qall{s}{\IfBooleanTF{#1}{}{\quad}\text{all}\quad}
\DeclareDocumentCommand\qeven{s}{\IfBooleanTF{#1}{}{\quad}\text{even}\quad}
\DeclareDocumentCommand\qodd{s}{\IfBooleanTF{#1}{}{\quad}\text{odd}\quad}
\DeclareDocumentCommand\qinteger{s}{\IfBooleanTF{#1}{}{\quad}\text{integer}\quad}
\DeclareDocumentCommand\qand{s}{\IfBooleanTF{#1}{}{\quad}\text{and}\quad}
\DeclareDocumentCommand\qor{s}{\IfBooleanTF{#1}{}{\quad}\text{or}\quad}
\DeclareDocumentCommand\qas{s}{\IfBooleanTF{#1}{}{\quad}\text{as}\quad}
\DeclareDocumentCommand\qin{s}{\IfBooleanTF{#1}{}{\quad}\text{in}\quad}
\DeclareDocumentCommand\qcc{s}{\IfBooleanTF{#1}{}{\quad}\text{c.c.}\quad}

% Derivatives
\DeclareDocumentCommand\differential{ o g d() }{ % Differential 'd'
	% o: optional n for nth differential
	% g: optional argument for readability and to control spacing
	% d: long-form as in d(cos x)
	\IfNoValueTF{#2}{
		\IfNoValueTF{#3}
			{\diffd\IfNoValueTF{#1}{}{^{#1}}}
			{\mathinner{\diffd\IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
		}
		{\mathinner{\diffd\IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
	}
\DeclareDocumentCommand\dd{}{\differential} % Shorthand for \differential

\DeclareDocumentCommand\derivative{ s o m g d() }
{ % Total derivative
	% s: star for \flatfrac flat derivative
	% o: optional n for nth derivative
	% m: mandatory (x in df/dx)
	% g: optional (f in df/dx)
	% d: long-form d/dx(...)
	\IfBooleanTF{#1}
	{\let\fractype\flatfrac}
	{\let\fractype\frac}
	\IfNoValueTF{#4}
	{
		\IfNoValueTF{#5}
		{\fractype{\diffd \IfNoValueTF{#2}{}{^{#2}}}{\diffd #3\IfNoValueTF{#2}{}{^{#2}}}}
		{\fractype{\diffd \IfNoValueTF{#2}{}{^{#2}}}{\diffd #3\IfNoValueTF{#2}{}{^{#2}}} \argopen(#5\argclose)}
	}
	{\fractype{\diffd \IfNoValueTF{#2}{}{^{#2}} #3}{\diffd #4\IfNoValueTF{#2}{}{^{#2}}}}
}
\DeclareDocumentCommand\dv{}{\derivative} % Shorthand for \derivative

\DeclareDocumentCommand\partialderivative{ s o m g g d() }
{ % Partial derivative
	% s: star for \flatfrac flat derivative
	% o: optional n for nth derivative
	% m: mandatory (x in df/dx)
	% g: optional (f in df/dx)
	% g: optional (y in d^2f/dxdy)
	% d: long-form d/dx(...)
	\IfBooleanTF{#1}
	{\let\fractype\flatfrac}
	{\let\fractype\frac}
	\IfNoValueTF{#4}
	{
		\IfNoValueTF{#6}
		{\fractype{\partial \IfNoValueTF{#2}{}{^{#2}}}{\partial #3\IfNoValueTF{#2}{}{^{#2}}}}
		{\fractype{\partial \IfNoValueTF{#2}{}{^{#2}}}{\partial #3\IfNoValueTF{#2}{}{^{#2}}} \argopen(#6\argclose)}
	}
	{
		\IfNoValueTF{#5}
		{\fractype{\partial \IfNoValueTF{#2}{}{^{#2}} #3}{\partial #4\IfNoValueTF{#2}{}{^{#2}}}}
		{\fractype{\partial^2 #3}{\partial #4 \partial #5}}
	}
}
\DeclareDocumentCommand\pderivative{}{\partialderivative} % Shorthand for \partialderivative
\DeclareDocumentCommand\pdv{}{\partialderivative} % Shorthand for \partialderivative

\DeclareDocumentCommand\variation{ o g d() }{ % Functional variation
	% o: optional n for nth differential
	% g: optional argument for readability and to control spacing
	% d: long-form as in d(F(g))
	\IfNoValueTF{#2}{
		\IfNoValueTF{#3}
			{\delta \IfNoValueTF{#1}{}{^{#1}}}
			{\mathinner{\delta \IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
		}
		{\mathinner{\delta \IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
	}
\DeclareDocumentCommand\var{}{\variation} % Shorthand for \variation

\DeclareDocumentCommand\functionalderivative{ s o m g d() }
{ % Functional derivative
	% s: star for \flatfrac flat derivative
	% o: optional n for nth derivative
	% m: mandatory (g in dF/dg)
	% g: optional (F in dF/dg)
	% d: long-form d/dx(...)
	\IfBooleanTF{#1}
	{\let\fractype\flatfrac}
	{\let\fractype\frac}
	\IfNoValueTF{#4}
	{
		\IfNoValueTF{#5}
		{\fractype{\variation \IfNoValueTF{#2}{}{^{#2}}}{\variation #3\IfNoValueTF{#2}{}{^{#2}}}}
		{\fractype{\variation \IfNoValueTF{#2}{}{^{#2}}}{\variation #3\IfNoValueTF{#2}{}{^{#2}}} \argopen(#5\argclose)}
	}
	{\fractype{\variation \IfNoValueTF{#2}{}{^{#2}} #3}{\variation #4\IfNoValueTF{#2}{}{^{#2}}}}
}
\DeclareDocumentCommand\fderivative{}{\functionalderivative} % Shorthand for \functionalderivative
\DeclareDocumentCommand\fdv{}{\functionalderivative} % Shorthand for \functionalderivative

% Bra-ket notation
\DeclareDocumentCommand\bra{ s m t\ket s g }
{ % Bra
	\IfBooleanTF{#3}
	{ % Contraction
		\IfBooleanTF{#1}
		{ % Bra has a star: no resize
			\IfNoValueTF{#5}
			{\braket*{#2}{} \IfBooleanTF{#4}{*}{}}
			{\braket*{#2}{#5}}
		}
		{
			\IfBooleanTF{#4}
			{ % Ket has a star: no resize
				\IfNoValueTF{#5}
				{\braket{#2}{} *}
				{\braket*{#2}{#5}}
			}
			{\braket{#2}{\IfNoValueTF{#5}{}{#5}}} % Neither term is starred: auto sizing
		}
	}
	{ % No contraction
		\IfBooleanTF{#1}
		{\vphantom{#2}\left\langle\smash{#2}\right\rvert}
		{\left\langle{#2}\right\rvert}
		\IfBooleanTF{#4}{*}{}
		\IfNoValueTF{#5}{}{#5}
	}
}

\DeclareDocumentCommand\ket{ s m }
{ % Ket
	\IfBooleanTF{#1}
	{\vphantom{#2}\left\lvert\smash{#2}\right\rangle} % No resize
	{\left\lvert{#2}\right\rangle} % Auto sizing
}

\DeclareDocumentCommand\innerproduct{ s m g }
{ % Inner product
	\IfBooleanTF{#1}
	{ % No resize
		\IfNoValueTF{#3}
		{\vphantom{#2}\left\langle\smash{#2}\middle\vert\smash{#2}\right\rangle}
		{\vphantom{#2#3}\left\langle\smash{#2}\middle\vert\smash{#3}\right\rangle}
	}
	{ % Auto resize
		\IfNoValueTF{#3}
		{\left\langle{#2}\middle\vert{#2}\right\rangle}
		{\left\langle{#2}\middle\vert{#3}\right\rangle}
	}
}
\DeclareDocumentCommand\braket{}{\innerproduct} % Alternative for \innerproduct
\DeclareDocumentCommand\ip{}{\innerproduct} % Shorthand for \innerproduct
	
\DeclareDocumentCommand\outerproduct{ s m g }
{ % Dyad
	\IfBooleanTF{#1}
	{ % No resize
		\IfNoValueTF{#3}
		{\vphantom{#2}\left\lvert\smash{#2}\middle\rangle\!\middle\langle\smash{#2}\right\rvert}
		{\vphantom{#2#3}\left\lvert\smash{#2}\middle\rangle\!\middle\langle\smash{#3}\right\rvert}
	}
	{ % Auto resize
		\IfNoValueTF{#3}
		{\left\lvert{#2}\middle\rangle\!\middle\langle{#2}\right\rvert}
		{\left\lvert{#2}\middle\rangle\!\middle\langle{#3}\right\rvert}
	}
}
\DeclareDocumentCommand\dyad{}{\outerproduct} % Alternative for \outerproduct
\DeclareDocumentCommand\op{}{\dyad} % Shorthand for \outerproduct
\DeclareDocumentCommand\ketbra{}{\dyad} % Alternative for \outerproduct

\DeclareDocumentCommand\expectationvalue{ s s m g }
{ % Expectation value
	\IfNoValueTF{#4}
	{
		\IfBooleanTF{#1}
		{\vphantom{#3}\left\langle\smash{#3}\right\rangle} % Starred implicit form: no resizing
		{\left\langle{#3}\right\rangle} % Normal implicit form: auto sizing
	}
	{
		\IfBooleanTF{#1}
		{
			\IfBooleanTF{#2}
			{\left\langle{#4}\middle\vert{#3}\middle\vert{#4}\right\rangle} % Double starred explicit form: total auto sizing
			{\vphantom{#3#4}\left\langle\smash{#4}\middle\vert\smash{#3}\middle\vert\smash{#4}\right\rangle} % Starred explicit form: no resizing
		}
		{\vphantom{#3}\left\langle{#4}\middle\vert\smash{#3}\middle\vert{#4}\right\rangle} % Normal explicit form: only resize based on bra/ket arguments
	}
}
\DeclareDocumentCommand\expval{}{\expectationvalue} % Shorthand for \expectationvalue
\DeclareDocumentCommand\ev{}{\expectationvalue} % Shorthand for \expectationvalue
\DeclareDocumentCommand\vev{ m }{\expectationvalue{#1}{0}} % Vacuum expectation value

\DeclareDocumentCommand\matrixelement{ s s m m m }
{ % Matrix element
	\IfBooleanTF{#1}
	{
		\IfBooleanTF{#2}
		{\left\langle{#3}\middle\vert{#4}\middle\vert{#5}\right\rangle} % Double starred: total resizing
		{\vphantom{#3#4#5}\left\langle\smash{#3}\middle\vert\smash{#4}\middle\vert\smash{#5}\right\rangle} % Starred: no resizing
	}
	{\vphantom{#4}\left\langle{#3}\middle\vert\smash{#4}\middle\vert{#5}\right\rangle} % Normal: only resize based on bra/ket arguments
}
\DeclareDocumentCommand\matrixel{}{\matrixelement} % Shorthand for \matrixelement
\DeclareDocumentCommand\mel{}{\matrixelement} % Shorthand for \matrixelement

% Matrix macros
\DeclareDocumentCommand\identitymatrix{m}
{
	{
		\newtoks\matrixtoks
		\global\matrixtoks = {}
		\newcount\rowcount
		\newcount\colcount
		\loop
		\colcount = 0
		\advance \rowcount by 1
		{
			\loop
			\advance \colcount by 1
			\edef\addtoks
			{
				\ifnum \colcount = 1 \else & \fi
				\ifnum \colcount = \rowcount 1 \else 0 \fi
			}
			\global\matrixtoks = \expandafter{\the\expandafter\matrixtoks\addtoks}
			\ifnum \colcount < #1
			\repeat
		}
		\ifnum \rowcount < #1
			\global\matrixtoks = \expandafter{\the\matrixtoks \\ }
			\repeat
	}
	\the\matrixtoks
}
\DeclareDocumentCommand\imat{}{\identitymatrix}

\DeclareDocumentCommand\xmatrix{ s m m m }
{
	{
		\newtoks\matrixtoks
		\global\matrixtoks = {}
		\newcount\rowcount
		\newcount\colcount
		\loop
		\colcount = 0
		\advance \rowcount by 1
		{
			\loop
			\advance \colcount by 1
			\edef\addtoks{\ifnum \colcount = 1 \else & \fi #2 \IfBooleanTF{#1}{_{\ifnum #3 > 1 \the\rowcount \fi \ifnum #4 > 1 \the\colcount \fi}}{}}
			\global\matrixtoks = \expandafter{\the\expandafter\matrixtoks\addtoks}
			\ifnum \colcount < #4
			\repeat
		}
		\ifnum \rowcount < #3
			\global\matrixtoks = \expandafter{\the\matrixtoks \\ }
			\repeat
	}
	\the\matrixtoks
}
\DeclareDocumentCommand\xmat{}{\xmatrix}

\DeclareDocumentCommand\zeromatrix{ m g }{\IfNoValueTF{#2}{\xmatrix{0}{#1}{#1}}{\xmatrix{0}{#1}{#2}}}
\DeclareDocumentCommand\zmat{}{\zeromatrix}

\DeclareDocumentCommand\paulixmatrix{}{0&1\\1&0}
\DeclareDocumentCommand\pauliymatrix{}{0&-i\\i&0}
\DeclareDocumentCommand\paulizmatrix{}{1&0\\0&-1}
\DeclareDocumentCommand\paulimatrix{m}
{
	\let\argin=#1
	\ifx\argin 0 \identitymatrix{2} \else
	\ifx\argin 1 \paulixmatrix \else
	\ifx\argin 2 \pauliymatrix \else
	\ifx\argin 3 \paulizmatrix \else
	\ifx\argin x \paulixmatrix \else
	\ifx\argin y \pauliymatrix \else
	\ifx\argin z \paulizmatrix \fi\fi\fi\fi\fi\fi\fi
}
\DeclareDocumentCommand\pmat{}{\paulimatrix}

\DeclareDocumentCommand\diagonalmatrix{O{} >{\SplitList{,}}m }{\@dmat{#1}#2}
\DeclareDocumentCommand\@dmat{mmggggggg}
{
	\newtoks\matrixtoks
	\global\matrixtoks = {}
	\IfNoValueTF{#3}
	{#2}
	{
		\IfNoValueTF{#4}
		{\global\matrixtoks = \expandafter{\mqty{#2}&#1\\#1&\mqty{#3}}}
		{
			\IfNoValueTF{#5}
			{\global\matrixtoks = \expandafter{\mqty{#2}&#1&#1\\#1&\mqty{#3}&#1\\#1&#1&\mqty{#4}}}
			{
				\IfNoValueTF{#6}
				{\global\matrixtoks = \expandafter{\mqty{#2}&#1&#1&#1\\#1&\mqty{#3}&#1&#1\\#1&#1&\mqty{#4}&#1\\#1&#1&#1&\mqty{#5}}}
				{
					\IfNoValueTF{#7}
					{\global\matrixtoks = \expandafter{\mqty{#2}&#1&#1&#1&#1\\#1&\mqty{#3}&#1&#1&#1\\#1&#1&\mqty{#4}&#1&#1\\#1&#1&#1&\mqty{#5}&#1\\#1&#1&#1&#1&\mqty{#6}}}
					{
						\IfNoValueTF{#8}
						{\global\matrixtoks = \expandafter{\mqty{#2}&#1&#1&#1&#1&#1\\#1&\mqty{#3}&#1&#1&#1&#1\\#1&#1&\mqty{#4}&#1&#1&#1\\#1&#1&#1&\mqty{#5}&#1&#1\\#1&#1&#1&#1&\mqty{#6}&#1\\#1&#1&#1&#1&#1&\mqty{#7}}}
						{
							\IfNoValueTF{#9}
							{\global\matrixtoks = \expandafter{\mqty{#2}&#1&#1&#1&#1&#1&#1\\#1&\mqty{#3}&#1&#1&#1&#1&#1\\#1&#1&\mqty{#4}&#1&#1&#1&#1\\#1&#1&#1&\mqty{#5}&#1&#1&#1\\#1&#1&#1&#1&\mqty{#6}&#1&#1\\#1&#1&#1&#1&#1&\mqty{#7}&#1\\#1&#1&#1&#1&#1&#1&\mqty{#8}}}
							{\global\matrixtoks = \expandafter{\mqty{#2}&#1&#1&#1&#1&#1&#1&#1\\#1&\mqty{#3}&#1&#1&#1&#1&#1&#1\\#1&#1&\mqty{#4}&#1&#1&#1&#1&#1\\#1&#1&#1&\mqty{#5}&#1&#1&#1&#1\\#1&#1&#1&#1&\mqty{#6}&#1&#1&#1\\#1&#1&#1&#1&#1&\mqty{#7}&#1&#1\\#1&#1&#1&#1&#1&#1&\mqty{#8}&#1\\#1&#1&#1&#1&#1&#1&#1&\mqty{#9}}}
						}
					}
				}
			}
		}
	}
	\the\matrixtoks
}
\DeclareDocumentCommand\dmat{}{\diagonalmatrix}

\DeclareDocumentCommand\antidiagonalmatrix{O{} >{\SplitList{,}}m }{\@admat{#1}#2}
\DeclareDocumentCommand\@admat{mmggggggg}
{
	\newtoks\matrixtoks
	\global\matrixtoks = {}
	\IfNoValueTF{#3}
	{#2}
	{
		\IfNoValueTF{#4}
		{\global\matrixtoks = \expandafter{#1&\mqty{#2}\\\mqty{#3}&#1}}
		{
			\IfNoValueTF{#5}
			{\global\matrixtoks = \expandafter{#1&#1&\mqty{#2}\\#1&\mqty{#3}&#1\\\mqty{#4}&#1&#1}}
			{
				\IfNoValueTF{#6}
				{\global\matrixtoks = \expandafter{#1&#1&#1&\mqty{#2}\\#1&#1&\mqty{#3}&#1\\#1&\mqty{#4}&#1&#1\\\mqty{#5}&#1&#1&#1}}
				{
					\IfNoValueTF{#7}
					{\global\matrixtoks = \expandafter{#1&#1&#1&#1&\mqty{#2}\\#1&#1&#1&\mqty{#3}&#1\\#1&#1&\mqty{#4}&#1&#1\\#1&\mqty{#5}&#1&#1&#1\\\mqty{#6}&#1&#1&#1&#1}}
					{
						\IfNoValueTF{#8}
						{\global\matrixtoks = \expandafter{#1&#1&#1&#1&#1&\mqty{#2}\\#1&#1&#1&#1&\mqty{#3}&#1\\#1&#1&#1&\mqty{#4}&#1&#1\\#1&#1&\mqty{#5}&#1&#1&#1\\#1&\mqty{#6}&#1&#1&#1&#1\\\mqty{#7}&#1&#1&#1&#1&#1}}
						{
							\IfNoValueTF{#9}
							{\global\matrixtoks = \expandafter{#1&#1&#1&#1&#1&#1&\mqty{#2}\\#1&#1&#1&#1&#1&\mqty{#3}&#1\\#1&#1&#1&#1&\mqty{#4}&#1&#1\\#1&#1&#1&\mqty{#5}&#1&#1&#1\\#1&#1&\mqty{#6}&#1&#1&#1&#1\\#1&\mqty{#7}&#1&#1&#1&#1&#1\\\mqty{#8}&#1&#1&#1&#1&#1&#1}}
							{\global\matrixtoks = \expandafter{#1&#1&#1&#1&#1&#1&#1&\mqty{#2}\\#1&#1&#1&#1&#1&#1&\mqty{#3}&#1\\#1&#1&#1&#1&#1&\mqty{#4}&#1&#1\\#1&#1&#1&#1&\mqty{#5}&#1&#1&#1\\#1&#1&#1&\mqty{#6}&#1&#1&#1&#1\\#1&#1&\mqty{#7}&#1&#1&#1&#1&#1\\#1&\mqty{#8}&#1&#1&#1&#1&#1&#1\\\mqty{#9}&#1&#1&#1&#1&#1&#1&#1}}
						}
					}
				}
			}
		}
	}
	\the\matrixtoks
}
\DeclareDocumentCommand\admat{}{\antidiagonalmatrix}

% Misc
\DeclareDocumentCommand\flatfrac{ m m }{\left.#1\middle\slash#2\right.}
\DeclareDocumentCommand\homework{}{ % You can try it
	\ensuremath{
	\div{\vb{E}}=\frac{\rho}{\epsilon_0} \qc
	\div{\vb{B}}=0 \qc
	\curl{\vb{E}}=-\pdv{\vb{B}}{t}\qc
	\curl{\vb{B}}=\mu_0\vb{J}+\frac{1}{c^2}\pdv{\vb{E}}{t}\qc
	H\ket{\Psi}=i\hbar\pdv{}{t}\ket{\Psi},
	\qq{all else follows.}
	}
}
